Impact of Annealing and Nanostructuring on Properties of NV Centers Created by Different Techniques

Nitrogen-vacancy (NV) centers in diamonds have been an epicenter of research for diverse applications in quantum technologies. It is therefore imperative that their fabrication techniques are well understood and characterized for the technological scalability of these applications. A comparative study of the optical and spin properties of NVs created by ion implantation and chemical vapor deposition delta-doping is thus presented, combined with an investigation on the impact of annealing in vacuum at different temperatures. In addition, nanopillars are fabricated with electron beam lithography and reactive ion etching for enhanced photon collection efficiency. An extensive combination of characterization techniques is employed. Notably, the smallest nanopillars present fluorescence enhancements of factor around 50, compared to the unstructured regions. Annealing is also demonstrated to increase the optical contrast between the NVs' electronic states, the coherence and relaxation times both in bulk as in pillars. Regarding the NV preparation technique, the delta-doping is shown to create NVs with less lattice defects and strain compared to implantation.

==> latexmkrc <==
$sub_doc_output = 'output-subdoc';

@sub_doc_options = ();

push @sub_doc_options, '-pdf'; # Use pdflatex for compilation of external documents.
# Replace '-pdf' by '-pdfdvi', 'pdfxe', or 'pdflua' if needed.

push @file_not_found, '^No file\\s*(.+)\s*$';

add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );
sub makeexternaldocument {
    if ( $root_filename ne $_[0] )  {
        my ($base_name, $path) = fileparse( $_[0] );
        pushd $path;
        my $return = system "latexmk",
                            @sub_doc_options,
                            "-aux-directory=$sub_doc_output",
                            "-output-directory=$sub_doc_output",
                            $base_name;
        if ( ($sub_doc_output ne '') && ($sub_doc_output ne '.') ) {

             rdb_add_generated( "$sub_doc_output/$base_name.aux" );
             copy "$sub_doc_output/$base_name.aux", ".";
        }
        popd;
        return $return;
   }
}
